Towards Generating Adversarial Examples on Mixed-type Data

The existence of adversarial attacks (or adversarial examples) brings huge concern about the machine learning (ML) model's safety issues. For many safety-critical ML tasks, such as financial forecasting, fraudulent detection, and anomaly detection, the data samples are usually mixed-type, which contain plenty of numerical and categorical features at the same time. However, how to generate adversarial examples with mixed-type data is still seldom studied. In this paper, we propose a novel attack algorithm M-Attack, which can effectively generate adversarial examples in mixed-type data. Based on M-Attack, attackers can attempt to mislead the targeted classification model's prediction, by only slightly perturbing both the numerical and categorical features in the given data samples. More importantly, by adding designed regularizations, our generated adversarial examples can evade potential detection models, which makes the attack indeed insidious. Through extensive empirical studies, we validate the effectiveness and efficiency of our attack method and evaluate the robustness of existing classification models against our proposed attack. The experimental results highlight the feasibility of generating adversarial examples toward machine learning models in real-world applications.

==> section/unused.tex <==



%\par In this section, we present the experimental results of our proposed M-attack and the baseline model on the home Credit Dataset, IEEE-CIS transaction dataset, and Criteo Display Advertising Dataset. The target model to attack on these two dataset are MLPs. In each dataset, we conduct 16 groups of experiments with $\epsilon_1$ equals {0.1, 0.3, 0.6, 0.9}, and $\epsilon_2$ equals {1, 2, 3, 4} respectively, and for each configuration of $\epsilon_1$ and $\epsilon_2$, a group of 10 experiments are conducted, and the results presented in this section are averaged in each group.

%\textbf{{Results on Home Credit Dataset.}} Table.\ref{tab:loan1} shows the results on Home Credit Dataset. From the results of the SR, we can see that our proposed M-Attack can achieve competitive performance as the baseline model, which also illustrates that our proposed M-Attack can generate adversarial examples effectively. Meanwhile, by inspecting the average time of generating an adversarial example, our proposed M-Attack has significant advantage over the baseline. And as $\epsilon_2$ increases, the advantage becomes larger, which can reach $\textbf{81\%}$ reduction on time comparing with the baseline. This improvement on efficiency is quite significant.


\begin{table}[t]
\centering
\caption{M-Attack vs.PGD+Greedy on Home Credit Dataset}
\resizebox{0.4\textwidth}{!}
{
\begin{tabular}{c| cc|cc } 
\hline\hline
 &   \multicolumn{2}{c|}{\textbf{M-Attack}} 
 & \multicolumn{2}{c}{\textbf{PGD+Greedy}}
\\
\hline
&SR. & Time &SR. & Time \\
\hline
\textbf{$\epsilon_1 = 0.1$, $\epsilon_2 = 1$.} & 0.33 & 4.670 & 0.385 & 4.973\\ 
\textbf{$\epsilon_1 = 0.1$, $\epsilon_2 = 2$.} & 0.595 & 3.149 & 0.610 & 3.549\\ 
\textbf{$\epsilon_1 = 0.1$, $\epsilon_2 = 3$.} & 0.755 & 2.375 & 0.780 & 3.206\\ 
\textbf{$\epsilon_1 = 0.1$, $\epsilon_2 = 4$.} & 0.850 & 2.122 & 0.875 & 2.337\\ 
 \hline
\textbf{$\epsilon_1 = 0.3$, $\epsilon_2 = 1$.} & 0.44 & 3.729 & 0.535 & 4.015\\ 
\textbf{$\epsilon_1 = 0.3$, $\epsilon_2 = 2$.} & 0.725 & 2.338 & 0.74 & 2.731\\ 
\textbf{$\epsilon_1 = 0.3$, $\epsilon_2 = 3$.} & 0.835 & 1.798 & 0.865 & 2.613\\ 
\textbf{$\epsilon_1 = 0.3$, $\epsilon_2 = 4$.} & 0.890 & 1.702 & 0.91 & 4.808\\ 
\hline
\textbf{$\epsilon_1 = 0.6$, $\epsilon_2 = 1$.} & 0.605 & 3.526 & 0.685 & 3.875\\ 
\textbf{$\epsilon_1 = 0.6$, $\epsilon_2 = 2$.} & 0.835 & 2.025 & 0.870 & 2.476\\ 
\textbf{$\epsilon_1 = 0.6$, $\epsilon_2 = 3$.} & 0.905 & 1.643 & 0.920 & 2.595\\ 
\textbf{$\epsilon_1 = 0.6$, $\epsilon_2 = 4$.} & 0.925 & 1.515 & 0.965 & 5.066\\ 
\hline
\textbf{$\epsilon_1 = 0.9$, $\epsilon_2 = 1$.} & 0.73 & 2.348 & 0.845 & 2.647\\ 
\textbf{$\epsilon_1 = 0.9$, $\epsilon_2 = 2$.} & 0.890 & 1.460 & 0.935 & 1.866\\ 
\textbf{$\epsilon_1 = 0.9$, $\epsilon_2 = 3$.} & 0.915 & 1.249 & 0.965 & 2.078\\ 
\textbf{$\epsilon_1 = 0.9$, $\epsilon_2 = 4$.} & 0.945 & 1.348 & 0.995 & 4.848 \\ 
\hline
\end{tabular}}
\label{tab:loan1}
\end{table}

\textbf{{Results on IEEE-CIS transaction Dataset.}} Similar to the results on Home Credit Default Risk dataset, our proposed M-Attack can achieve competitive performance as the baseline model, which also illustrates that our proposed M-Attack can generate adversarial examples effectively. Meanwhile, our proposed M-Attack has significant advantage over the baseline. And as $\epsilon_2$ increases, the advantage becomes larger. This improvement on efficiency is quite significant.

\textbf{{Results on Criteo Display Advertising Challenge dataset.}} Similar to the results on Home Credit Default Risk dataset and IEEE-CIS transaciton dataset, our proposed M-Attack can achieve competitive performance as the baseline model, which also illustrates that our proposed M-Attack can generate adversarial examples effectively. Meanwhile, our proposed M-Attack has significant advantage over the baseline. And as $\epsilon_2$ increases, the advantage becomes larger. This improvement on efficiency is quite significant.

